Kwai Keye-VL 1.5 Technical Report

In recent years, the development of Large Language Models (LLMs) has significantly advanced, extending their capabilities to multimodal tasks through Multimodal Large Language Models (MLLMs). However, video understanding remains a challenging area due to the dynamic and information-dense nature of videos. Existing models struggle with the trade-off between spatial resolution and temporal coverage when processing video content. We present Keye-VL-1.5, which addresses fundamental challenges in video comprehension through three key innovations. First, we introduce a novel Slow-Fast video encoding strategy that dynamically allocates computational resources based on inter-frame similarity, processing key frames with significant visual changes at higher resolution (Slow pathway) while handling relatively static frames with increased temporal coverage at lower resolution (Fast pathway). Second, we implement a progressive four-stage pre-training methodology that systematically extends the model's context length from 8K to 128K tokens, enabling processing of longer videos and more complex visual content. Third, we develop a comprehensive post-training pipeline focusing on reasoning enhancement and human preference alignment, incorporating a 5-step chain-of-thought data construction process, iterative GSPO-based reinforcement learning with progressive prompt hinting for difficult cases, and alignment training. Through extensive evaluation on public benchmarks and rigorous internal human assessment, Keye-VL-1.5 demonstrates significant improvements over existing models, particularly excelling in video understanding tasks while maintaining competitive performance on general multimodal benchmarks.

==> arXiv/cases/auto_yes.tex <==
\subsubsubsection{Thinking Case}
\renewcommand{\arraystretch}{1.5}
\begin{figure}[!h]
  \centering
  \begin{tabular}{m{16cm}}
  \toprule
  \begin{center}
  Input Image
  \end{center}
  \begin{center}
  \includegraphics[width=0.5\linewidth]{arXiv/cases/figs/auto_yes.jpg}
  \end{center}
  \\
  {\footnotesize \textbf{Prompts:} Find x.\newline\newline
  \textbf{Model Responses:} 
 \texttt{<analysis>}
 This question involves calculating the area of a shaded region formed by two semicircles, where specific geometric properties and relationships between the semicircles and the chord are given. This requires understanding the geometry and performing calculations to determine the area. Therefore, /think mode is more appropriate.\texttt{</analysis>}
 
\texttt{ <think>}The problem that users need to solve now is the area of the shaded region. First, it is necessary to understand the composition of the figure: the shaded region should be the area of the larger semicircle minus the area of the smaller semicircle, or the area of the larger semicircle minus the area of the smaller semicircle plus the area of the smaller semicircle? No, looking at the figure, the shaded region is the part of the larger semicircle excluding the smaller semicircle, so it is the area of the larger semicircle minus the area of the smaller semicircle. Then, it is necessary to find the radii of the larger and smaller semicircles.

First, let the radius of the larger semicircle be R and the radius of the smaller semicircle be r. Since CD is parallel to AB and CD touches the smaller semicircle, the distance from the center O of the larger semicircle to CD is equal to the radius r of the smaller semicircle. The length of CD is 4, so in the right triangle formed by half of CD, the radius R of the larger semicircle, and the distance r, according to the Pythagorean theorem, we have (CD/2)² + r² = R², which is 2² + r² = R², i.e., 4 + r² = R².

Then, the area of the shaded region is the area of the larger semicircle minus the area of the smaller semicircle, which is 
$\frac{1}{2}\pi R^2 - \frac{1}{2}\pi r^2 = \frac{1}{2}\pi (R^2 - r^2)$. From the previous equation,
$R^2 - r^2 = 4$, 
so the area is $\frac{1}{2}\pi \times 4 = 2\pi$. Thus, the area of the shaded region is $2\pi$.\texttt{</think>}

\texttt{<answer>}
To solve this problem, we can analyze the area of the shaded region by combining the Pythagorean theorem and the formula for the area of a circle.

Step 1: Define Variables and Analyze Geometric Relationships
Let the radius of the larger semicircle be ( R ) and the radius of the smaller semicircle be ( r ). Observing the figure, we know that the chord ( CD ) is parallel to the diameter ( AB ) of the larger semicircle and is tangent to the smaller semicircle. Therefore, the distance from the center ( O ) of the larger semicircle to ( CD ) is equal to the radius ( r ) of the smaller semicircle.

The length of ( CD ) is 4, so half of ( CD ) is ( $\frac{CD}{2} = 2$ ). At this point, a right triangle can be formed: one leg is ( $\frac{CD}{2} = 2$ ), the other leg is the distance from the center ( O ) to ( CD ) (i.e., ( r )), and the hypotenuse is the radius ( R ) of the larger semicircle.

Step 2: Use the Pythagorean Theorem to Find ( $R^2 - r^2$ )
According to the Pythagorean theorem, in the right triangle, we have: [ $\left( \frac{CD}{2} \right)^2 + r^2 = R^2$ ] Substituting ( $\frac{CD}{2} = 2$ ), we get: [ $2^2 + r^2 = R^2 \implies 4 + r^2 = R^2 \implies R^2 - r^2 = 4$ ]

Step 3: Calculate the Area of the Shaded Region
The area of the shaded region is equal to the area of the larger semicircle minus the area of the smaller semicircle. According to the formula for the area of a circle ( $S = \pi r^2$ ), the area of the semicircle is ( $\frac{1}{2} \pi r^2$ ). Therefore: [ \text{Area of the shaded region} = $\frac{1}{2} \pi R^2 - \frac{1}{2} \pi r^2 = \frac{1}{2} \pi (R^2 - r^2)$ ] Substituting ( $R^2 - r^2 = 4 $), we get: [ \text{Area of the shaded region} = $\frac{1}{2} \pi \times 4 = 2\pi$ ]

In conclusion, the area of the shaded region is ($\boxed{2\pi}$).
\texttt{</answer>}
  }
  \\
  \bottomrule
  \end{tabular}
\caption{An example demonstrating Kwai Keye-VL choosing the Thinking mode to solve a hard geometry problem.}
\label{fig:think}
\end{figure}
\renewcommand{\arraystretch}{1}

\clearpage

